Dialectal Toxicity Detection: Evaluating LLM-as-a-Judge Consistency Across Language Varieties

There has been little systematic study on how dialectal differences affect toxicity detection by modern LLMs. Furthermore, although using LLMs as evaluators ("LLM-as-a-judge") is a growing research area, their sensitivity to dialectal nuances is still underexplored and requires more focused attention. In this paper, we address these gaps through a comprehensive toxicity evaluation of LLMs across diverse dialects. We create a multi-dialect dataset through synthetic transformations and human-assisted translations, covering 10 language clusters and 60 varieties. We then evaluated three LLMs on their ability to assess toxicity across multilingual, dialectal, and LLM-human consistency. Our findings show that LLMs are sensitive in handling both multilingual and dialectal variations. However, if we have to rank the consistency, the weakest area is LLM-human agreement, followed by dialectal consistency. Code repository: \url{https://github.com/ffaisal93/dialect_toxicity_llm_judge}

==> app_content.tex <==
\begin{table}[ht]
\small
    % \centering
    \begin{tabular}{l|l}
    \toprule
     Section & Desctiption \\
     \midrule
     \cref{app:rel_work} & Related Work \\
     \cmidrule{1-2}
     \multirow{2}{*}{\cref{sec:tasks_benchmark}}    & Tasks of \benchmark\\
     & \tabitem Translate-Test NLI Dataset Statistics (\cref{{tab:nli_data}}) \\

    \cmidrule{1-2}
      \multirow{3}{*}{\cref{app:lang_stdv}} &  \Dialects{} and \Clusters{} of \benchmark \\
     & \tabitem \benchmark{} \Dialect{} list (\cref{lang_list})\\
     & \tabitem Language \Clusters{} and Representative \Dialects{} (\cref{stdv})\\

     \cmidrule{1-2}
     \multirow{18}{*}{\cref{app:plots}} & Result Visualizations\\ \\
     & 
     
    \begin{tabular}{l}
        Regional maps with aggregated Machine Translation scores (\crefrange{fig:swiss_german_mt}{fig:italian_mt})\\
        \cmidrule{1-1}
         \tabitem Map of Switzerland with aggregated BLEU scores of Swiss-German variety per region (\cref{fig:swiss_german_mt}) \\
         \tabitem Map of Italy with aggregated BLEU scores of Italian variety per region (\cref{fig:italian_mt}) \\\\

         Task Specific Plot for Maximum Scores (\crefrange{fig:plot_app_1}{fig:plot_app_4})\\
        \cmidrule{1-1}
         \tabitem Parts-of-Speech Tagging (\cref{fig:pos}) \\
        \tabitem Named entity recognition (\cref{fig:ner})\\
        
        \tabitem Topic classification  (\cref{fig:tc})\\
        \tabitem Natural language inference (\cref{fig:nli})\\
        
        \tabitem Extractive question answering (\cref{fig:qa})\\
        \tabitem Multiple-choice machine reading comprehension (\cref{fig:rcmc})\\
        \tabitem Sentiment analysis (\cref{fig:sc})\\
        \tabitem Dialect identification (\cref{fig:di}) \\%\DC{Somehow I find this one hard to remember. DID or DId?}
        
        
        \tabitem Machine translation (MT-region) (\cref{fig:mt-region})\\
        \tabitem Machine translation (MT-dialect) (\cref{fig:mt-dialect})\\
        
        \\

        Dialectal Gap visualization  utilizing zero-shot cross-lingual transfer from Standard English.\\
        \cmidrule{1-1}
        \tabitem Parts-of-Speech Tagging (\cref{fig:pos-gap})\\
        \tabitem Named entity recognition (\cref{fig:ner-gap})\\
        \tabitem Dialect identification (\cref{fig:nli-gap})\\
    \end{tabular}\\

    \cmidrule{1-2}
     \multirow{11}{*}{\cref{app:detailed_result_tables}} & Task Specific Evaluation Result Tables\\ 
     & 
    \begin{tabular}{l}
        \cmidrule{1-1}
        \tabitem Dependency parsing (\cref{tab:dep_full}) \\
         \tabitem Parts-of-Speech tagging (\cref{tab:pos_full}) \\
        \tabitem Named entity recognition (\cref{tab:ner_full})\\
        \tabitem Natural language inference (\cref{tab:nli})\\
        \tabitem Extractive question answering (\crefrange{tab:sdqa_dev}{tab:sdqa_test})\\
        
        \tabitem Dialect identification (\cref{tab:id_all}) \\
        \tabitem Topic classification  (\cref{tab:topic})\\
        \tabitem Sentiment analysis (\cref{tab:sc})\\
        
        \tabitem Multiple-choice machine reading comprehension (\cref{tab:mrc})\\
        
        \tabitem Machine translation (\cref{zero-shot-mt})\\
    \end{tabular}\\

    \cmidrule{1-2}
    \cref{app:high_low} & Highest performing and lowest performing varieties (\cref{{tab:high-lang}}) \\

    \cmidrule{1-2}
    \cref{app:non_std_zeroshot} & Low-resource \Dialect{} performing better in zero-shot NER (\cref{tab:script}) \\
    
    \cmidrule{1-2}
     \cref{app:c_summary}    & \Cluster{} level Result Summaries with Demographic Utility and Standard Deviation report (\crefrange{tab:summery-DEP. Parsing}{tab:summery-EQA})\\

     \cmidrule{1-2}
     \cref{sec:icl_prompts} & In-Context Learning Details \\
     
    \bottomrule
    \end{tabular}
    \caption{Table of contents for supplementary material.}
    \label{tab:app_content}
\end{table}



==> compare_gap.tex <==
\begin{table}[t]
\centering
\tiny
\begin{tabular}{@{}p{.8cm}l@{}r|r|r}
\toprule
Task & Gap metric                         &  Avg. val &             \cluster{} (max)&               \cluster{} (min)\\
\midrule
\multirow{3}{*}{DEP parsing} & $\gapiii{\text{eng}}{\text{eng}}{C}$ &      34.0 &   arabic, 50.8 &  sw. shift. romance, 19.4 \\
      & $\gapiii{\text{eng}}{\std{v}}{C}$ &      15.7 &   anglic, 34.2 &  sw. shift. romance, $-0.9$ \\
      & $\gapiii{\text{in-variety}}{\std{v}}{C}$ &      26.4 &   arabic, 93.8 &                italian romance, 0.6 \\
\cmidrule{1-5}
\multirow{3}{*}{POS tagging} & $\gapiii{\text{eng}}{\text{eng}}{C}$ &      27.4 &   arabic, 58.5 &                     norwegian, 14.7 \\
      & $\gapiii{\text{eng}}{\std{v}}{C}$ &       6.7 &   anglic, 20.9 &      ew. armenian, $-2.1$ \\
      & $\gapiii{\text{in-variety}}{\std{v}}{C}$ &       6.2 &   arabic, 29.1 &                          neva, $-0.5$ \\
\cmidrule{1-5}
\multirow{3}{*}{NER} & $\gapiii{\text{eng}}{\text{eng}}{C}$ &      31.7 &  kurdish, 77.1 &                  modern dutch, 12.3 \\
      & $\gapiii{\text{eng}}{\std{v}}{C}$ &      22.3 &  kurdish, 78.2 &                   hindustani, $-23.6$ \\
      & $\gapiii{\std{v}}{\std{v}}{C}$ &     $-28.6$ &  kurdish, 91.5 &                    sorbian, -1162.7 \\
\cmidrule{1-5}
% \multirow{3}{*}{EQA} & $\gapiii{\text{eng}}{\text{eng}}{C}$ &      43.8 &   korean, 89.8 &                         anglic, 1.6 \\
%       & $\gapiii{\text{eng}}{\std{v}}{C}$ &       0.1 &    anglic, 1.6 &                       bengali, $-1.6$ \\
%       & $\gapiii{\mathcal{L}}{\std{v}}{C}$ &       3.3 &  swahili, 12.1 &                       bengali, $-1.9$ \\
% \cmidrule{1-5}
\multirow{3}{*}{TC} & $\gapiii{\text{eng}}{\text{eng}}{C}$ &      22.4 &  kurdish, 74.2 &                        sinitic, 0.4 \\
      & $\gapiii{\text{eng}}{\std{v}}{C}$ &      12.5 &  kurdish, 60.6 &                     norwegian, $-2.2$ \\
      & $\gapiii{\std{v}}{\std{v}}{C}$ &      $-1.9$ &  latvian, 21.0 &                      kurdish, $-61.3$ \\
\bottomrule
\end{tabular}
\caption{Comparative cluster-level dialectal gap across tasks. In general, the average disparity is larger for zero-shot transfer $\gapiii{\text{eng}}{\text{eng}}{C}$. However, when we 
move from zeroshot to finetune (i.e. $\mathcal{G}_{\text{eng}}\rightarrow\mathcal{G}_{\bar{v}/\text{in-variety}}$) and compute the distance from a \cluster{} representative $\std{v}$, we observe increased dialectal disparity $|\gapiii{}{\std{v}}{C}|$.}
\label{tab:compare_gap}
\end{table}

==> task_dataset.tex <==
\begin{table*}[!t]
    \centering
    \tiny
    \begin{tabular}{@{}p{1.2cm}|p{1.5cm}@{}p{.8cm}p{1cm}@{}p{1cm}p{9cm}@{}}
    \toprule
    Category & Task & Metric &\#Clusters&\#Varieties & Source Dataset \\
    \midrule
     Structured Prediction
     &POS tagging&F1&11&25&Universal Dependency~\cite{11234/1-4611}, Singlish~\cite{wang-etal-2017-universal-fixed}\\
     \midrule
     Classification& DId & F1 &6&45& MADAR~\cite{bouamor-etal-2018-madar}, DMT~\cite{jauhiainen-etal-2019-discriminating}, Greek~\cite{8554709}, DSL-TL~\cite{zampieri2023language}, Swiss Germans~\cite{articleswiss}\\
     &SA&F1&1&9&TSAC~\cite{medhaffar-etal-2017-sentiment},
TUNIZI~\cite{fourati-etal-2021-introducing},
DzSentiA~\cite{9068897},
SaudiBank~\cite{alqahtani-etal-2022-customer},
 MAC~\cite{Garouani_MAC},
 ASTD~\cite{nabil-etal-2015-astd},
AJGT~\cite{10.1007/978-3-319-60042-0_66},
OCLAR~\cite{8716394} \\
&TC & F1 &15&38& SIB-200~\cite{adelani2023sib200}\\
&NLI& F1 &15&38& XNLI~\cite{conneau-etal-2018-xnli} translate-test\\
\midrule
Question & MRC& F1 &4&11& Belebele~\cite{bandarkar2023belebele}\\
Answering& EQA& Span F1 &5&24&SDQA~\cite{faisal-etal-2021-sd-qa}\\
  \bottomrule
    \end{tabular}
   \caption{Subset of \benchmark{} tasks used to evaluate generative models against multilingual encoders. This table presents selected dialectal and variety-specific datasets, highlighting task metrics, number of language clusters, and varieties. The study extends the original benchmark to compare instruction-tuned LLM performance with traditional multilingual models.}
    \label{tab:task}
\end{table*}
